Joint Lemmatization and Morphological Tagging with LEMMING

We present LEMMING, a modular log-linear model that jointly models lemmatization and tagging and supports the integration of arbitrary global features. It is trainable on corpora annotated with gold standard tags and lemmata and does not rely on morphological dictionaries or analyzers. LEMMING sets the new state of the art in token-based statistical lemmatization on six languages; e.g., for Czech lemmatization, we reduce the error by 60%, from 4.05 to 1.58. We also give empirical evidence that jointly modeling morphological tags and lemmata is mutually beneficial.

==> tables/dev.tex <==
\begin{tabular}{l@{\hskip 4pt}llrrrrrrrrrrrr}
&&& \multicolumn{2}{c}{cs} & \multicolumn{2}{c}{de} & \multicolumn{2}{c}{en} & \multicolumn{2}{c}{es} & \multicolumn{2}{c}{hu} & \multicolumn{2}{c}{la} \\
\hline
\multirow{15}{*}{\begin{sideways}{\Large Baselines}\end{sideways}}
& \sw{simple} & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 87.22 & 32.95 & 93.27 & 62.15 & 97.60 & 75.64 & 92.92 & 59.68 & 86.09 & 42.02 & 85.19 & 14.06 \\
&  & joint & 77.18 & 22.56 & 75.60 & 36.43 & 93.15 & 67.58 & 90.28 & 54.00 & 82.99 & 37.03 & 75.00 & 5.39 \\
\cline{2-15}
& \sw{simple} & tag & \ul{89.82} & \ul{76.83} & \ul{85.05} & \ul{65.22} & \ul{\tb{95.71}} & \ul{\tb{90.29}} & \ul{96.83} & \ul{89.00} & \ul{\tb{95.46}} & \ul{88.17} & \ul{86.35} & \ul{65.21} \\
& \marmot & lemma & 87.36 & 32.95 & 93.28 & 62.15 & 97.66 & 75.64 & 92.99 & 59.68 & 86.11 & 42.02 & 85.35 & 14.06 \\
&  & joint & 79.99 & 23.98 & 80.71 & 40.26 & 94.09 & 69.48 & 90.75 & 54.66 & 83.47 & 37.16 & 76.58 & 6.61 \\
\cline{2-15}
& JCK & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 96.24 & 82.59 & 97.67 & 88.80 & 98.71 & 92.50 & 97.61 & 86.76 & 97.48 & 91.16 & \ul{93.26} & \ul{63.09} \\
&  & joint & 84.32 & 61.67 & 78.10 & 51.42 & 94.43 & 84.61 & 94.67 & 78.39 & 93.15 & 80.73 & 81.34 & 43.71 \\
\cline{2-15}
& JCK & tag & \ul{89.82} & \ul{76.83} & \ul{85.05} & \ul{65.22} & \ul{\tb{95.71}} & \ul{\tb{90.29}} & \ul{96.83} & \ul{89.00} & \ul{\tb{95.46}} & \ul{88.17} & \ul{86.35} & \ul{65.21} \\
& \marmot & lemma & \ul{96.26} & \ul{82.88} & \ul{97.74} & 89.11 & \ul{98.81} & \ul{93.06} & 97.78 & 87.10 & \ul{97.68} & \ul{91.91} & 93.06 & 62.64 \\
&  & joint & \ul{88.17} & \ul{68.43} & \ul{84.16} & \ul{60.39} & \ul{95.41} & \ul{86.95} & \ul{95.37} & 80.25 & \ul{94.33} & \ul{83.70} & \ul{83.57} & \ul{48.84} \\
\cline{2-15}
& \sw{morfette} & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 96.25 & 82.54 & 97.12 & \ul{89.90} & 98.43 & 92.54 & \ul{97.97} & \ul{89.94} & 97.22 & 90.04 & 91.89 & 55.13 \\
&  & joint & 84.39 & 61.94 & 77.60 & 52.87 & 94.16 & 84.70 & 95.09 & \ul{81.95} & 93.11 & 80.60 & 80.09 & 36.39 \\
\hline
\hline
\multirow{27}{*}{\begin{sideways}{\Large \software{lemming}}\end{sideways}}
& edit tree & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 96.29 & 82.93 & 97.84 & 89.78 & 98.71 & 92.63 & 97.91 & 89.00 & 97.31 & 90.49 & 93.00 & 61.68 \\
&  & joint & 84.45 & 62.36 & 78.32 & 52.75 & 94.43 & 84.79 & 94.97 & 80.68 & 93.08 & 80.48 & 80.92 & 41.27 \\
\cline{2-15}
& align & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 96.74 & 85.38 & 98.17 & 91.61 & 98.76 & 93.11 & 98.05 & 90.13 & 97.70 & 92.15 & 93.76 & 66.30 \\
&  & joint & 84.72 & 63.88 & 78.47 & 53.52 & 94.47 & 85.09 & 95.05 & 81.29 & 93.31 & 81.51 & 81.49 & 44.67 \\
\cline{2-15}
& dict & tag & 86.08 & 69.83 & 79.05 & 56.02 & 94.72 & 87.95 & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 97.50 & 89.38 & 98.36 & 92.66 & 98.84 & 94.02 & 98.39 & 92.56 & 97.98 & 93.30 & 94.64 & 71.57 \\
&  & joint & 85.06 & 65.60 & 78.53 & 53.91 & 94.53 & 85.83 & 95.27 & 82.89 & 93.46 & 82.10 & 81.87 & 46.92 \\
\cline{2-15}
& morph & tag & 86.08 & 69.83 & 79.05 & 56.02 & \NA & \NA & 96.29 & 87.21 & 94.37 & 85.20 & 83.86 & 57.77 \\
& \sw{morfette} & lemma & 96.59 & 87.28 & 97.43 & 89.96 & \NA & \NA & 98.46 & 92.98 & 97.77 & 92.62 & 93.60 & 66.30 \\
&  & joint & 85.64 & 67.73 & 78.87 & 55.17 & \NA & \NA & 95.63 & 84.69 & 94.10 & 84.02 & 82.29 & 48.72 \\
\cline{2-15}
& edit tree & tag & 89.82 & 76.83 & 85.05 & 65.22 & \tb{95.71} & \tb{90.29} & 96.83 & 89.00 & \tb{95.46} & 88.17 & 86.35 & 65.21 \\
& \marmot & lemma & 96.33 & 83.04 & 97.93 & 90.05 & 98.82 & 93.02 & 98.14 & 89.61 & 97.53 & 91.22 & 92.85 & 60.98 \\
&  & joint & 88.23 & 68.85 & 84.41 & 61.89 & 95.40 & 87.00 & 95.75 & 83.06 & 94.30 & 83.58 & 83.20 & 46.73 \\
\cline{2-15}
& align & tag & 89.82 & 76.83 & 85.05 & 65.22 & \tb{95.71} & \tb{90.29} & 96.83 & 89.00 & \tb{95.46} & 88.17 & 86.35 & 65.21 \\
& \marmot & lemma & 96.80 & 85.72 & 98.24 & 91.94 & 98.88 & 93.71 & 98.27 & 90.75 & 97.91 & 92.91 & 93.50 & 64.89 \\
&  & joint & 88.57 & 70.69 & 84.59 & 62.95 & 95.45 & 87.47 & 95.81 & 83.64 & 94.52 & 84.60 & 83.83 & 50.32 \\
\cline{2-15}
& dict & tag & 89.82 & 76.83 & 85.05 & 65.22 & \tb{95.71} & \tb{90.29} & 96.83 & 89.00 & \tb{95.46} & 88.17 & 86.35 & 65.21 \\
& \marmot & lemma & 97.62 & 89.88 & 98.43 & 92.95 & 98.94 & \tb{94.28} & 98.62 & 93.23 & 98.23 & 94.16 & 94.49 & 70.60 \\
&  & joint & 88.97 & 72.79 & 84.63 & 63.16 & \tb{95.50} & \tb{88.08} & 96.02 & 85.24 & 94.73 & 85.46 & 84.41 & 53.79 \\
\cline{2-15}
& morph & tag & 89.82 & 76.83 & 85.05 & 65.22 & \NA & \NA & 96.83 & 89.00 & \tb{95.46} & 88.17 & 86.35 & 65.21 \\
& \marmot & lemma & 97.38 & 89.55 & 98.24 & 92.42 & \NA & \NA & \tb{98.71} & 93.97 & 98.30 & 94.38 & 94.39 & 70.54 \\
&  & joint & 89.30 & 74.32 & 84.81 & 64.08 & \NA & \NA & 96.17 & 86.29 & 95.15 & 86.87 & 84.62 & 55.07 \\
\cline{2-15}
& dict & tag & \tb{90.47} & 78.37 & 85.31 & 65.94 & 95.66 & 88.60 & 96.94 & 89.25 & 95.29 & 87.55 & \tb{86.77} & 65.98 \\
& joint & lemma & 98.34 & 92.96 & 98.66 & 94.07 & \tb{99.00} & 94.23 & 98.68 & 94.08 & 98.53 & 95.46 & \tb{96.68} & \tb{82.99} \\
&  & joint & 89.82 & 75.47 & 84.94 & 64.19 & 95.48 & 86.52 & 96.11 & 85.43 & 94.71 & 85.40 & 85.85 & 60.98 \\
\cline{2-15}
& morph & tag & 90.35 & \tb{79.61} & \tb{85.52} & \tb{67.69} & 95.66 & 88.60 & \tb{96.95} & \tb{89.55} & \tb{95.46} & \tb{88.85} & 86.70 & \tb{66.82} \\
& joint & lemma & \tb{98.55} & \tb{94.12} & \tb{98.74} & \tb{94.47} & \tb{99.00} & 94.23 & 98.68 & \tb{94.53} & \tb{98.57} & \tb{95.65} & 96.51 & 82.22 \\
&  & joint & \tb{90.05} & \tb{78.37} & \tb{85.28} & \tb{66.58} & 95.48 & 86.52 & \tb{96.20} & \tb{86.51} & \tb{95.30} & \tb{88.22} & \tb{85.97} & \tb{62.97} \\
\end{tabular}


==> tables/tst.tex <==
\begin{tabular}{l@{\hskip 4pt}llrrrrrrrrrrrr}
&&& \multicolumn{2}{c}{cs} & \multicolumn{2}{c}{de} & \multicolumn{2}{c}{en} & \multicolumn{2}{c}{es} & \multicolumn{2}{c}{hu} & \multicolumn{2}{c}{la} \\
\hline
\multirow{15}{*}{\begin{sideways}{\Large Baselines}\end{sideways}}
& \sw{simple} & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 86.81 & 31.16 & 91.42 & 58.68 & 97.88 & 78.95 & 92.86 & 59.34 & 84.67 & 38.95 & 83.60 & 20.43 \\
&  & joint & 76.96 & 21.22 & 72.83 & 33.27 & 93.82 & 68.98 & 90.14 & 53.45 & 80.41 & 33.08 & 71.62 & 7.52 \\
\cline{2-15}
& \sw{simple} & tag & \ul{89.75} & \ul{76.83} & \ul{82.81} & \ul{61.60} & \ul{\tb{96.45}} & \ul{\tb{90.68}} & \ul{97.05} & \ul{90.07} & \ul{93.64} & \ul{84.65} & \ul{82.37} & \ul{53.73} \\
& \marmot & lemma & 86.94 & 31.16 & 91.48 & 58.68 & 97.92 & 78.95 & 92.92 & 59.34 & 84.73 & 38.95 & 83.80 & 20.43 \\
&  & joint & 79.66 & 22.86 & 77.78 & 36.49 & 94.87 & 71.62 & 90.81 & 54.98 & 81.06 & 33.27 & 73.51 & 8.58 \\
\cline{2-15}
& JCK & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 95.87 & 80.79 & 96.50 & 85.54 & 98.95 & 93.76 & 97.58 & 86.80 & 96.52 & 88.09 & \ul{90.84} & 58.13 \\
&  & joint & 84.00 & 59.46 & 75.60 & 47.77 & 95.09 & 84.34 & 94.54 & 77.97 & 90.71 & 75.62 & 76.76 & 33.56 \\
\cline{2-15}
& JCK & tag & \ul{89.75} & \ul{76.83} & \ul{82.81} & \ul{61.60} & \ul{\tb{96.45}} & \ul{\tb{90.68}} & \ul{97.05} & \ul{90.07} & \ul{93.64} & \ul{84.65} & \ul{82.37} & \ul{53.73} \\
& \marmot & lemma & \ul{95.95} & \ul{81.28} & \ul{96.63} & 85.84 & \ul{99.08} & \ul{94.28} & 97.69 & 87.19 & \ul{96.69} & \ul{88.66} & 90.79 & \ul{58.23} \\
&  & joint & \ul{87.85} & \ul{67.00} & \ul{81.60} & \ul{55.97} & \ul{96.17} & \ul{87.32} & \ul{95.44} & 80.62 & \ul{92.15} & \ul{78.89} & \ul{79.51} & \ul{39.07} \\
\cline{2-15}
& \sw{morfette} & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 95.88 & 80.70 & 95.88 & \ul{87.55} & 98.73 & 93.56 & \ul{98.02} & \ul{90.16} & 96.06 & 86.21 & 90.08 & 54.16 \\
&  & joint & 84.10 & 59.92 & 74.87 & 49.22 & 94.89 & 84.44 & 95.03 & \ul{81.68} & 90.60 & 75.11 & 76.57 & 32.50 \\
\hline
\hline
\multirow{27}{*}{\begin{sideways}{\Large \software{lemming}}\end{sideways}}
& edit tree & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 95.91 & 81.07 & 96.82 & 87.31 & 98.95 & 93.69 & 97.87 & 88.97 & 96.15 & 86.68 & 91.20 & 59.87 \\
&  & joint & 84.15 & 60.27 & 75.86 & 49.22 & 95.08 & 84.37 & 94.86 & 80.38 & 90.50 & 74.86 & 77.00 & 34.73 \\
\cline{2-15}
& align & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 96.43 & 83.83 & 97.22 & 89.25 & 98.99 & 94.15 & 98.04 & 90.28 & 96.87 & 89.72 & 91.64 & 62.36 \\
&  & joint & 84.47 & 61.97 & 76.05 & 50.07 & 95.11 & 84.73 & 94.98 & 81.30 & 90.94 & 76.76 & 77.18 & 35.79 \\
\cline{2-15}
& dict & tag & 86.00 & 68.88 & 76.80 & 52.86 & 95.35 & 87.58 & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 97.24 & 88.13 & 97.58 & 91.03 & 99.07 & 95.06 & 98.32 & 92.36 & 97.28 & 91.32 & 92.97 & 69.14 \\
&  & joint & 84.88 & 64.14 & 76.13 & 50.48 & 95.19 & 85.55 & 95.19 & 82.91 & 91.14 & 77.48 & 77.52 & 37.59 \\
\cline{2-15}
& morph & tag & 86.00 & 68.88 & 76.80 & 52.86 & \NA & \NA & 96.30 & 87.65 & 92.33 & 81.32 & 79.70 & 47.06 \\
& \sw{morfette} & lemma & 96.52 & 86.69 & 96.57 & 88.26 & \NA & \NA & 98.53 & 93.73 & 96.70 & 89.30 & 91.53 & 62.31 \\
&  & joint & 85.57 & 66.73 & 76.56 & 51.90 & \NA & \NA & 95.63 & 85.02 & 91.92 & 79.73 & 78.18 & 39.65 \\
\cline{2-15}
& edit tree & tag & 89.75 & 76.83 & 82.81 & 61.60 & \tb{96.45} & \tb{90.68} & 97.05 & 90.07 & 93.64 & 84.65 & 82.37 & 53.73 \\
& \marmot & lemma & 96.05 & 81.68 & 96.99 & 87.69 & 99.08 & 94.25 & 98.00 & 89.56 & 96.38 & 87.54 & 91.37 & 60.88 \\
&  & joint & 88.03 & 68.04 & 81.96 & 57.91 & 96.17 & 87.38 & 95.80 & 83.42 & 91.93 & 78.15 & 79.75 & 40.34 \\
\cline{2-15}
& align & tag & 89.75 & 76.83 & 82.81 & 61.60 & \tb{96.45} & \tb{90.68} & 97.05 & 90.07 & 93.64 & 84.65 & 82.37 & 53.73 \\
& \marmot & lemma & 96.56 & 84.49 & 97.38 & 89.68 & 99.12 & 94.51 & 98.17 & 90.89 & 97.11 & 90.61 & 91.80 & 63.26 \\
&  & joint & 88.41 & 70.03 & 82.20 & 59.02 & 96.19 & 87.61 & 95.94 & 84.38 & 92.41 & 80.14 & 80.03 & 41.87 \\
\cline{2-15}
& dict & tag & 89.75 & 76.83 & 82.81 & 61.60 & \tb{96.45} & \tb{90.68} & 97.05 & 90.07 & 93.64 & 84.65 & 82.37 & 53.73 \\
& \marmot & lemma & 97.46 & 89.14 & 97.70 & 91.27 & \tb{99.21} & \tb{95.59} & 98.48 & 92.98 & 97.53 & 92.10 & 93.07 & 69.83 \\
&  & joint & 88.86 & 72.51 & 82.27 & 59.42 & \tb{96.27} & \tb{88.49} & 96.12 & 85.80 & 92.59 & 80.77 & 80.49 & 44.26 \\
\cline{2-15}
& morph & tag & 89.75 & 76.83 & 82.81 & 61.60 & \NA & \NA & 97.05 & 90.07 & 93.64 & 84.65 & 82.37 & 53.73 \\
& \marmot & lemma & 97.29 & 88.98 & 97.51 & 90.85 & \NA & \NA & 98.68 & 94.32 & 97.53 & 92.15 & 92.54 & 67.81 \\
&  & joint & 89.23 & 74.24 & 82.49 & 60.42 & \NA & \NA & 96.35 & 87.25 & 93.11 & 82.56 & 80.67 & 45.21 \\
\cline{2-15}
& dict & tag & \tb{90.34} & 78.47 & \tb{83.10} & 62.36 & 96.32 & 89.70 & 97.11 & 90.13 & 93.64 & 84.78 & 82.89 & 54.69 \\
& joint & lemma & 98.27 & 92.67 & \tb{98.10} & 92.79 & \tb{99.21} & 95.23 & 98.67 & 94.07 & 98.02 & 94.15 & \tb{95.58} & \tb{81.74} \\
&  & joint & 89.69 & 75.44 & 82.64 & 60.49 & 96.17 & 87.87 & 96.23 & 86.19 & 92.84 & 81.89 & 81.92 & 49.97 \\
\cline{2-15}
& morph & tag & 90.20 & \tb{79.72} & \tb{83.10} & \tb{63.10} & 96.32 & 89.70 & \tb{97.17} & \tb{90.66} & \tb{93.67} & \tb{85.12} & \tb{83.49} & \tb{58.76} \\
& joint & lemma & \tb{98.42} & \tb{93.46} & \tb{98.10} & \tb{93.02} & \tb{99.21} & 95.23 & \tb{98.78} & \tb{94.86} & \tb{98.08} & \tb{94.26} & 95.36 & 80.94 \\
&  & joint & \tb{89.90} & \tb{78.34} & \tb{82.84} & \tb{62.10} & 96.17 & 87.87 & \tb{96.41} & \tb{87.47} & \tb{93.40} & \tb{84.15} & \tb{82.57} & \tb{54.63} \\
\end{tabular}

